Optical Properties of Charged Defects in Monolayer MoS$_2$

We present theoretical calculations of the optical spectrum of monolayer MoS$_2$ with a charged defect. In particular, we solve the Bethe-Salpeter equation based on an atomistic tight-binding model of the MoS$_2$ electronic structure which allows calculations for large supercells. The defect is modelled as a point charge whose potential is screened by the MoS$_2$ electrons. We find that the defect gives rise to new peaks in the optical spectrum approximately 100-200 meV below the first free exciton peak. These peaks arise from transitions involving in-gap bound states induced by the charged defect. Our findings are in good agreement with experimental measurements.

==> old_text.tex <==

%% INTRO

% The weaker dielectric screening effect that is present in monolayer TMDCs, compared to in 3D bulk semiconductors, results in a stronger Coulomb interaction between electrons and holes which leads to large exciton binding energies \cite{Colloquium2018, berkelbach2018}. This has been shown in work by Li \emph{et al.} \cite{Li2014}, by extracting the imaginary part of the dielectric function through optical reflectance measurements for a handful of monolayer TMDCs (MoS$_2$, WS$_2$, MoSe$_2$, WSe$_2$) on fused silica substrates. This demonstrated that for these TMDCs, peaks appear at photon energies several hundreds of meV below the value of the quasi-particle band gap, which for MoS$_2$ on fused silica is found to be approximately 2.5 eV, and approximately 2.7 eV for WS$_2$ on fused silica \cite{Colloquium2018}. The lowest of the peaks corresponds to the optical band gap. The energy peaks in the imaginary part of the dielectric function appear to come in a pairs, more closely spaced in the case of the Mo-based TMDCs. These are referred to as the $A$ and $B$ excitons, and arise because of the strong spin-orbit splitting in the monolayer valence bands. This is known by comparing the separation between the $A$ and $B$ exciton to the spin-orbit splitting present in ab initio models or from ARPES \cite{Li2014, Colloquium2018}. This double peaked feature in the reflectance has also been observed in other work \cite{Splendiani2010}. The presence of two excitons with sizeable binding energy is also found when performing ab initio calculations. Calculations of the absorption spectrum and exciton resonances using the $GW$ method demonstrate how the weak screening in the material gives rise to larger binding energies \cite{qiu13}. These calculations are shown in Fig.~\ref{fig:intro_qiu_absorp}(a), where as well as the $A$ and $B$ exciton peaks of monolayer MoS$_2$, additional peaks are found in the band gap region that were not observed in experiment. This discrepancy is resolved when the broadening from quasi-particle lifetimes is included in the absorption spectrum, as seen in Fig.~\ref{fig:intro_qiu_absorp}(b).

% In TMDCs, the extent of the exciton wavefunction is on the order of several nanometres, with binding energy significantly less than that of a hydrogen atom, which is known as being within the Wannier-Mott regime \cite{Colloquium2018}. This is as opposed to the case of Frenkel excitons which have extents on the scale of the lattice parameter. Another unconventional property of TMDCs with respect to bulk semiconductors that manifests itself in the optical properties, is the large effective mass of the valley extrema ($\sim 0.5m_0$, where $m_0$ is the free electron mass). In a simple positronium model (electron + positron in free space) model for excitons in 2D, the lowest energy is proportional to the reduced mass $m_+m_-/(m_++m_-)$, where $m_{\pm}$ is the electron/hole mass (which for positronium, has $m_{\pm}=m_0$). This reduced mass in TMDCs, which evaluates to about $0.25m_0$, contributes to the unusually large binding energies of excitons. In the ab initio study of the optical properties of TMDCs by Qiu \emph{et al.} \cite{qiu13}, the character of the excitons is analysed and were compared to the bound states of the screened two-dimensional hydrogen model. The excitons corresponding to $A$ and $B$ resonances exhibited similar localised wavefunctions with a root mean square radius of 1 nanometre\cite{qiu13}. The $A$ and $B$ excitons were found to be doubly degenerate, because of the spin-valley locking present in the Brillouin zone, such that transitions for spin up electrons at $K$ are identical to spin down electrons at $K'$ \cite{Colloquium2018}. Additional exciton states were observed between the $B$ exciton and the quasi-particle band gap energy, which are labelled in Fig.~\ref{fig:intro_qiu_absorp}(a) as $A'$ and $B'$. These were found to be six-fold degenerate, and corresponded to $2s/2p$ states at the $K/K'$ points in the BZ \cite{qiu13}. 

% In addition to ab initio efforts to calculate properties of the excitons in monolayer TMDCs, tight-binding models can provide a quick and efficient means of describing the behaviour of excitons. In work by MacDonald \emph{et al.} \cite{Wu2015}, the Bethe-Salpeter equation was solved for a simple $4d$-orbital tight-binding model to obtain exciton binding energies of MoS$_2$ on SiO$_2$ substrate, which agree with experimentally obtained values. In contrast to Qiu \emph{et al.} \cite{qiu13}, in which the $GW$ calculations provided an accurate picture of the screening through the dielectric matrix of MoS$_2$, the screening was modelled using the Keldysh function. The inability of the two-dimensional Keldysh-screened Coulomb potential $V_{\mathbf{R}}$, given as a function of position $\mathbf{R}$, to accurately capture the electron-hole interaction at sub-nanometre scales was avoided through the truncation of the interaction. For $\mathbf{R}=0$, MacDonald sets the value of the interaction to be $UV_{\mathbf{R}=a}$ where $a$ is the lattice parameter and $U$ is an adjustable parameter that accounts for the screening of on-site potentials by remote bands, which takes unit value for the calculation (despite an uncertainty on its actual value). The optical conductivity from this approach exhibits similar features to the absorption obtained from both $GW$ calculations and reflectance experiments, namely a strongly bound exciton with binding energy on the order of a few hundred meV, and two dominant peaks at the lowest part of the spectrum corresponding to the $A$ and $B$ excitons \cite{Wu2015}. Overall, it can be seen that such a technique is capable of modelling optical properties of monolayer TMDC systems with significantly less computational cost than ab initio $GW$ calculations.

%  Point defects in the TMDC crystal can act as traps for excitons, which lead to light emission at energies lower than the optical band gap\cite{Tongay2012}. In work by Chow \emph{et al.}\cite{Chow2015}, monolayer MoS$_2$ and WS$_2$ were bombarded via argon plasma treatment over time, and the photoluminescence (PL) of the sample was measured. The bombardment caused vacancy defects which resulted in doping when exposed to air, causing a rise in the defect population over time. The PL exhibits a very strong peak occurring at time $t=0$ s corresponding to the first excited state of neutral excitons that occur in the pristine system, labelled at $X_O$. Additionally at $t=0$ s, a peak (labelled as $X_T$) forms that corresponds to charged excitons, known as trions, that are known to occur in heavily excited systems and doped systems.  It was deduced from comparison to studies of the defect free sample, that a defect peak arises from the bombardment of TMDCs causing radiative defect states that trap excitons\cite{Chow2015}.
 
%  In the work of Tongay \emph{et al.} \cite{Tongay2012}, MoS$_2$, MoSe$_2$ and WSe$_2$ were irradiated with alpha-particles (He$^{2+}$) to attain desired concentrations of point defects in the presence of N$_2$ gas. Similarly, they observe transitions from charged excitons to neutral excitons, which is explained as resulting from the charge depletion associated with the irradiation. The interaction of N$_2$ with the defect sites causes this charge depletion, which stabilises the neutral excitons and destabilises the trions\cite{Tongay2012}. As the defect concentration is enhanced by irradiation, the authors observe that a peak occurs with lower energy than both the charged and the neutral excitonic resonances, attributed to the radiative recombination of excitons that are bound to the created defects. The origin of these defects is inferred to be the interaction of defect sites with the N$_2$ gas because the observed bound excitonic resonances vanish upon purging of the N$_2$ gas\cite{Tongay2012}. The N$_2$, inert in the absence of vacancies in the TMDC, interacts with the chalcogen vacancies caused by irradiation, resulting in a small charge transfer from the TMDC to the N$_2$. The discrete defect states that arise from this interaction (which the authors have determined using supplementary first-principles calculations), are believed to be the source of multiple transitions to/from the conduction and valence bands near the band gap of the TMDC\cite{Tongay2012}.
 
%  In these experiments, different conclusions have arose when deducing the origin of the low-energy excitonic resonances that occur in the PL spectra. While the work of Tongay \emph{et al.} (vacuum + N$_2$) suggests possible transitions between defect states, Chow \emph{et al.} (ambient air: O$_2$, N$_2$, H$_2$O etc) suggest that such transitions are not occurring in their experiments, while the strong defect potential traps the excitons. Both observe the conversion between charged and neutral excitons, indicating that the interaction with surrounding gas acts to dope the system, depleting charge. Although these two effects could arise from different sources of point defects, the effects of the nature of the charged defect may prove to be interesting in the discussion. With different interacting chemicals, the charge transfer may differ between defect species, resulting in transitions to/from defect states that play roles of different importance in the optical spectrum. Thus, a greater understanding of how charged defects interplay with the excitonic features will provide insight to groups that observe such phenomena in PL experiments. This motivates study of how the optical absorption and binding energy of the excitons are modified by the external field caused by a charged defect.

%% METHODS


%In the basis of the centre-of-mass motion $\mathbf{R}$ and the relative motion $\mathbf{r}$, this is described by the expressions:
% \begin{align}
% 	\mathbf{r} =\mathbf{r}_e-\mathbf{r}_h & \longrightarrow \mathbf{r}_e = \mathbf{R} + \frac{m_h}{M}\mathbf{r},\\ 
% 	\mathbf{R}=\frac{m_e\mathbf{r}_e+m_h\mathbf{r}_h}{M}&\longrightarrow\, \;\;\;\mathbf{r}_h = \mathbf{R} - \frac{m_e}{M}\mathbf{r},
% \end{align}
% where $M=m_e+m_h$. 
% Substituting this into the Hamiltonian and using $\mathbf{p} = \hbar\mathbf{k}$, one obtains \cite{roessler}:
% \begin{equation}
% 	H_{e-h} = E_g - \frac{\hbar^2}{2\mu}\nabla^2 +V_{\text{scr}}(r)+ \frac{\hbar^2Q^2}{2M}
% \end{equation}

% where $\mu=\frac{m_em_h}{M}$ and $-i\nabla$ has been used as the real-space operator of $k$. The last term in $H_{e-h}$ vanishes for direct transitions with $Q=|\mathbf{Q}|=0$. It should also be noted that the momentum of the hole $\mathbf{p}_h$ has an opposite sign to that of the valence band electron that it replaces, while the position of the hole has the same sign as that from the corresponding valence band electron. In the case of monolayer TMDCs, this resembles the 2D hydrogen model more closely in energy level multiplicity and ordering, while deviating significantly from the analytic solution on account of the unique dielectric screening present in the material. 

% Excitons are the bound state of an electron and a hole, and the inclusion of such states into the optical conductivity requires the solution to the two-particle problem of the attractive interaction between a valence hole and a conduction electron \cite{Wu2015}. 

% Excitons are bound states of the quasi-particles formed when light is imparted onto a material, emerging from the mutual Coulomb attraction between an electron excited into the conduction band from the absorption of light, and the corresponding hole that is left in the valence band upon excitation. 

%For the case of direct transitions, where $Q=0$, the exchange integral is zero.

% In work by MacDonald \emph{et al.} \cite{Wu2015}, the Keldysh interaction is used to represent the interaction potential between the electron excited into the conduction band, and the hole in the valence band left behind. Typically, samples of TMDC in experiments are examined on a substrate which incurs a level of screening of the electron-hole charge. The screening included in the Keldysh interaction is the average of a silicon dioxide (SiO$_2$) substrate and air, $\varepsilon=2.4-2.5$.


%  The lattice Fourier transform $V_{\mathbf{q}}$ is represented on a grid spanned by vectors $\mathbf{R}_1=a\mathbf{\hat{x}}$ and $\mathbf{R}_2=(a/2)\mathbf{\hat{x}}+(\sqrt{3}a/2)\mathbf{\hat{y}}$, and has a size of $N_k\times N_k$. This is directly related to the $\mathbf{k}$ grid used to calculate the BSE Hamiltonian.


% A technique to reduce calculation time while retaining accuracy in the energy ranges of interest, involves limiting the number of transitions considered in the calculation between higher bands whose exciton energies are not greatly affected by the presence of charged defects. This is performed by introducing an energy cutoff $E_{\text{cut}}^{\text{BSE}}$, which determines the highest conduction band and lowest valence band considered in the calculation. 



% Due to the simplicity of the three-band model used in this work, the Hamiltonians corresponding to either spin can be decoupled from one another, meaning that if only the bright exciton states are required, the BSE can also be decoupled into same-spin transitions between either spin. However, the inclusion of exchange interactions will act to couple spin-up and spin-down transitions, such that the BSE can no longer be solved separately for each spin. The BSE already scales with supercell size $N_c$ to the fourth power, since it is proportional to the product of the number of conduction and valence bands.
